Robust Data-Driven Safe Control using Density Functions

This paper presents a tractable framework for data-driven synthesis of robustly safe control laws. Given noisy experimental data and some priors about the structure of the system, the goal is to synthesize a state feedback law such that the trajectories of the closed loop system are guaranteed to avoid an unsafe set even in the presence of unknown but bounded disturbances (process noise). The main result of the paper shows that for polynomial dynamics, this problem can be reduced to a tractable convex optimization by combining elements from polynomial optimization and the theorem of alternatives. This optimization provides both a rational control law and a density function safety certificate. These results are illustrated with numerical examples.

==> sections/SDDC.tex <==
This section presents the main results of the paper: a convex, tractable  reformulation of Problem 1.  In order to present these results, we begin by presenting  a tractable characterization of all systems that could have generated the observed data. 

Assume the sample data $\dc$ is corrupted by a sample (offline) noise bounded by $\epsilon$. The consistency set $\mathcal{P}_1$, 
which contains all systems that are consistent with the data, is defined as:


==> sections/abstract.tex <==
\begin{abstract} \label{sec:abstract}
% In this paper, we derive a data-driven method to design a robust safe controller for polynomial systems, using density functions as safety certificate. Two sets are defined in parameter space, one for compatible systems and one for safe systems. The inclusion of two sets is formulated as a polynomial feasibility problem. With the Sum-of-Squares (SOS) hierarchy, the problem is solved by Semidefinite Programming (SDP) solvers. Numerical examples are shown to illustrate the safety of closed-loop systems.
This paper performs data-driven synthesis of robustly safe control laws for polynomial dynamical systems using density functions. The resultant controllers are robust to process noise both during the learning process and during execution. Synthesis proceeds using a set-containment framework, in which the set of all consistent systems is certifiably contained within the set of all controller-secured systems using sum-of-squares nonnegativity proofs. Numerical examples are shown to illustrate the safety of closed-loop systems. 

\end{abstract}

==> sections/acknowledgements.tex <==
\section{Acknowledgements}

% \urg{Optional acknowledgements.}


==> sections/acronym.tex <==
\begin{acronym}
% \acro{BSA}{Basic Semialgebraic}
% \acro{DDC}{Data Driven Control}


% \acro{GAS}{Globally Asymptotically Stable}

\acro{CBF}{Control Barrier Function}

\acro{LMI}{Linear Matrix Inequality}
\acroplural{LMI}[LMIs]{Linear Matrix Inequalities}
\acroindefinite{LMI}{an}{a}
% \acp{LMI}: LMIs \iacf

\acro{LP}{Linear Program}
\acroindefinite{LP}{an}{a}
% \acro{OCP}{Optimal Control Problem}

% \acro{ODE}{Ordinary Differential Equation}

% \acro{POP}{Polynomial Optimization Problem}

% \acro{PSD}{Positive Semidefinite}

% \acro{PD}{Positive Definite}

% \acro{PDE}{Partial Differential Equation}

\acro{SDP}{Semidefinite Programming}
\acroindefinite{SDP}{an}{a}

\acro{SOS}{Sum of Squares}
\acroindefinite{SOS}{an}{a}
% \iac{} an SOS \Iac An SOS
% \acp

% \acro{WSOS}{Weighted Sum of Squares}

\end{acronym}

==> sections/introduction.tex <==
\section{Introduction} \ref{fig:ex1_nonrobust_no_noise}\label{sec:introduction}


This work finds safe full-state feedback control laws that are robust under $L_\infty$-bounded uncertainties in both data-collection and online dynamics (process noise). The \ac{DDC} problem over polynomial dynamics is posed as the feasibility of \iac{SOS} program. A density-function based control law may be derived from a feasible \ac{SDP} solution, thus certifying safety of all closed-loop trajectories with respect to a given initial and unsafe set. 

Trajectories starting from the initial set are safe if no point along the trajectories is ever inside the unsafe set. Level-set methods separate the initial and unsafe set by the $0$-contour of a solved function.
Barrier functions \cite{prajna2004safety} are a level set method to certify the safety of trajectories, given that the superlevel sets of the barrier function are invariant. This superlevel invariance can be relaxed through slack (class-K) conditions while ensuring that the $0$-level set is invariant \cite{ames2019control}. The level-set certificate of stability may be solved jointly with a safety-guaranteeing control policy $u(\cdot)$ (`control barrier function'). An alternative level-set certificate is  Density \cite{rantzer2004analysis} functions, which are based on Dual Lyapunov methods for stability \cite{rantzer2001dual}.   \urg{why choose Barrier vs Density? discuss here.} Other methods to ensure safety of controlled trajectories include funnels \cite{majumdar2013control}, Hamilton-Jacobi reachability \cite{bansal2017hamilton, chen2018hamilton}, Mixed Monotonicity \cite{coogan2020mixed}, and Reinforcement Learning \cite{brunke2022safe}.



% \urg{Literature review here.}


% \urg{Safe Control}

% \urg{Data-Driven Control, Data-Driven Safety}

\ac{DDC} is a methodology that formulates control laws directly from acquired system observations and skips a system-identification/robust-synthesis pipeline \cite{HOU20133, formentin2014comparison, hou2017datasurvey}. This paper utilizes a Set-Membership approach to \ac{DDC}: furnishing a control law $u(\cdot)$ with a certificate that the set of all data-consistent plants are contained within the set of all $u$-stabilized plants. The certificate in this work is expressed as \ac{SOS} nonnegativity proofs of linear inequalities over the basic-semialgebraic initial and unsafe sets \cite{parrilo2000structured}. Prior work that performs Set-Membership \ac{DDC} using \ac{SOS} proofs includes \cite{dai2020semi, martin2021data, miller2022eiv_short}. Other containment proofs used for Set-Membership \ac{DDC} include Farkas certificates for polytope containment \cite{cheng2015robust}, and a Matrix S-Lemma for Quadratic Matrix Inequalities \cite{waarde2020noisy}.
Other methods for \ac{DDC} include Iterative Feedback Tuning \cite{hjalmarsson1998iterative}, Virtual Reference Feedback Tuning \cite{campi2002virtual, formentin2012non}, Behavioral characterizations (Willem's Fundamental Lemma) \cite{willems2005note, depersis2020formulas, coulson2019data, berberich2021robustmpc}, and moment-based proofs for switching control  \cite{dai2018moments}.

Prior art for \ac{DDC} under safety constraints include \cite{rosolia2018learning, lopez2021robust, dacs2022robust}. To the best of our knowledge, our approach is the first \ac{DDC} method under safety constraints that simultaneously considers data-collection and online-dynamics noise.
% \vspace{-2cm}
% \urg{(outside of $H_2$ noise?)}.


% \urg{What makes our algorithm novel.}
\section{Introduction} \label{sec:introduction}


This work finds safe full-state feedback control laws that are robust under $L_\infty$-bounded uncertainties in both data-collection and online dynamics (process noise). The \ac{DDC} problem over polynomial dynamics is posed as the feasibility of \iac{SOS} program. A density-function based control law may be derived from a feasible \ac{SDP} solution, thus certifying safety of all closed-loop trajectories with respect to a given initial and unsafe set. 

Trajectories starting from the initial set are safe if no point along the trajectories is ever inside the unsafe set. Level-set methods separate the initial and unsafe set by the $0$-contour of a solved function.
Barrier functions \cite{prajna2004safety} are a level set method to certify the safety of trajectories, given that the superlevel sets of the barrier function are invariant. This superlevel invariance can be relaxed through slack (class-K) conditions while ensuring that the $0$-level set is invariant \cite{ames2019control}. The level-set certificate of stability may be solved jointly with a safety-guaranteeing control policy $u(\cdot)$ (`control barrier function'). An alternative level-set certificate is  Density \cite{rantzer2004analysis} functions, which are based on Dual Lyapunov methods for stability \cite{rantzer2001dual}.   \urg{why choose Barrier vs Density? discuss here.} Other methods to ensure safety of controlled trajectories include funnels \cite{majumdar2013control}, Hamilton-Jacobi reachability \cite{bansal2017hamilton, chen2018hamilton}, Mixed Monotonicity \cite{coogan2020mixed}, and Reinforcement Learning \cite{brunke2022safe}.



% \urg{Literature review here.}


% \urg{Safe Control}

% \urg{Data-Driven Control, Data-Driven Safety}

\ac{DDC} is a methodology that formulates control laws directly from acquired system observations and skips a system-identification/robust-synthesis pipeline \cite{HOU20133, formentin2014comparison, hou2017datasurvey}. This paper utilizes a Set-Membership approach to \ac{DDC}: furnishing a control law $u(\cdot)$ with a certificate that the set of all data-consistent plants are contained within the set of all $u$-stabilized plants. The certificate in this work is expressed as \ac{SOS} nonnegativity proofs of linear inequalities over the basic-semialgebraic initial and unsafe sets \cite{parrilo2000structured}. Prior work that performs Set-Membership \ac{DDC} using \ac{SOS} proofs includes \cite{dai2020semi, martin2021data, miller2022eiv_short}. Other containment proofs used for Set-Membership \ac{DDC} include Farkas certificates for polytope containment \cite{cheng2015robust}, and a Matrix S-Lemma for Quadratic Matrix Inequalities \cite{waarde2020noisy}.
Other methods for \ac{DDC} include Iterative Feedback Tuning \cite{hjalmarsson1998iterative}, Virtual Reference Feedback Tuning \cite{campi2002virtual, formentin2012non}, Behavioral characterizations (Willem's Fundamental Lemma) \cite{willems2005note, depersis2020formulas, coulson2019data, berberich2021robustmpc}, and moment-based proofs for switching control  \cite{dai2018moments}.

Prior art for \ac{DDC} under safety constraints include \cite{rosolia2018learning, lopez2021robust, dacs2022robust}. To the best of our knowledge, our approach is the first \ac{DDC} method under safety constraints that simultaneously considers data-collection and online-dynamics noise.
% \vspace{-2cm}
% \urg{(outside of $H_2$ noise?)}.


% \urg{What makes our algorithm novel.}
\begin{comment}
The goal of this paper is to develop a tractable framework for data-driven synthesis of safe control laws that are robust to $L_\infty$-bounded noise  in  data-collection and unknown but bounded disturbances during executions.
Trajectories starting from an initial set are safe if no point along the trajectories is ever inside the unsafe set. Level-set methods separate the initial and unsafe set by the $0$-contour of a solved function.
Barrier functions \cite{prajna2004safety} are a level set method to certify the safety of trajectories, given that the superlevel sets of the barrier function are invariant. This superlevel invariance can be relaxed through slack (class-K) conditions while ensuring that the $0$-level set is invariant \cite{ames2019control, xiao2019control}. The level-set certificate of stability may be solved jointly with a safety-guaranteeing control policy $u(\cdot)$ (`control barrier function'). When a barrier function is given, the min-norm controller will ensure safety of trajectories and can be found through quadratic programming \cite{freeman2008robust, ames2014control}. Robustness of given barrier functions to disturbances may be analyzed using input-to-state stability \cite{XU2015robustcbf}.
Barrier functions and funnels \cite{majumdar2013control} contain bilinearities when jointly synthesizing controllers and barriers.
An alternative level-set certificate is  Density \cite{rantzer2004analysis} functions, which are based on Dual Lyapunov methods for stability \cite{rantzer2001dual}. Controllers and density functions can be simultaneously solved for in a convex manner while also including input actuation constraints. Density functions may exist and provide improved performance as compared to  barrier functions in some systems \cite{chen2020densityvalue}.

We briefly compare against other methods of safety-constrained control.
Interval analyses such as Mixed Monotonicity \cite{coogan2020mixed} offer real-time performance at the expense of conservatism in safe generation.
Hamilton-Jacobi reachability \cite{bansal2017hamilton, chen2018hamilton} performs forward and backwards reachable set analysis based on level sets of a differential games' value function, whose computation could require solving PDEs or neural net approximations.
Reinforcement Learning necessitates training and prior information of safety properties (e.g. Lipschitz bounds on dynamics), and does not generally exploit physical principles and model structure \cite{brunke2022safe}. Koopman methods allow for predictive capabilities of nonlinear models \cite{korda2020optimal, otto2021koopman}, but they contain error bounds that can conflict against safety certification \cite{folkestad2020data}.

 \end{comment}

==> sections/methods.tex <==
\section{Data-Driven Safe Control} \label{sec:safe_no_w}


%%%-----------------------------
\subsection{Problem Statement}

% Consider the continuous-time control-affine system of the form
% \begin{equation} \label{eq:dynamics}
%     \dot{x} = f(x) + g(x) u
% \end{equation}
% where $x\in \R^n$ is the state, $u\in \R$ is the input, $f,g\colon \R^n \rightarrow \R^n$ are unknown polynomial functions, respectively. We assume the degrees of $f,g$ are known (or user-defined), then $f,g$ can be expressed by $f = F \phi$, $g = G \gamma$ where $F,G$ are unknown coefficient matrices and $\phi,\gamma$ are known monomial vectors in $x$, of proper dimensions. For example, for a two-state second-order polynomial system, $\phi,\gamma = [1,x_1,x_2,x_1^2,x_1x_2,x_2^2]^T$ and $F,G \in \R^{2\times 6}$.

The goal of this paper is to design a safe control law for a polynomial system where only system degrees and sample data are known. The problem is formally stated as:

\begin{problem} \label{pb:1}
Given an initial set $\mathcal{X}_0$ and an unsafe set $\mathcal{X}_u$ (both are basic semialgebraic), a noise bound $\epsilon > 0$, and noisy data $(y_s,x_s,u_s) = \dc$ generated by a system \eqref{eq:dynamics} under the relation that $\norm{y_s - f(x_s) - g(x_s) u_s}_\infty \leq \epsilon$, find a state-feedback control law $u(x)$ such that all systems consistent with data are safe w.r.t. $\mathcal{X}_0$ and $\mathcal{X}_u$.
\end{problem}

\begin{remark}
    The data $y_s$ is a noisy observation of the true derivative $\dot{x_s}$.
\end{remark}

\begin{remark}
The solved control law $u(x)$ is not necessarily consistent with sample data $\dc$.
\end{remark}

% In this section, we derive a data-driven algorithm to solve the problem \ref{pb:1}. 

The data-driven Problem \ref{pb:1} will be approached by  define two polytopic sets in parameter space: one for $\dc$-consistent systems ($\mathcal{P}_1$) and one for safe systems ($\mathcal{P}_2$). Applying the Extended Farkas' Lemma to enforce set-containment leads to a polynomial feasibility problem, which can be solved with \ac{SOS} method by \ac{SDP} solvers.

\subsection{Consistency Set}

Assume the sample data $\dc$ is corrupted by a sample (offline) noise bounded by $\epsilon$. The consistency set $\mathcal{P}_1$, 
which contains all systems that are consistent with the data, is defined as:
\begin{equation}
    \mathcal{P}_1 \doteq \left\{
    f,g\colon \|y_s-f(x_s)-g(x_s)u_s\|_\infty \leq \epsilon, t=1,\cdots,T \right\}.
\end{equation}
Recall that $f = F \phi$, $g = G \gamma$. By using the following property of the Kronecker product \cite{petersen2008matrix} $$\text{vec}(P^TXQ^T) = (Q\otimes P^T) \text{vec}(X),$$ an equivalent formulation is derived as
\begin{equation} \label{eq:p1}
    \mathcal{P}_1 = \left\{ 
    \mathbf{f},\mathbf{g} \colon 
    \begin{bmatrix}
        A & B \\ -A & -B
    \end{bmatrix} 
    \begin{bmatrix}
        \mathbf{f} \\ \mathbf{g}
    \end{bmatrix}
    \leq 
    \begin{bmatrix}
        \epsilon \mathbf{1} + \xi \\ \epsilon \mathbf{1} - \xi
    \end{bmatrix} \right\},
\end{equation}
where $\mathbf{f} = \text{vec} (F^T)$, $\mathbf{g} = \text{vec} (G^T)$ and
\begin{equation} \label{eq:abxi}
    A \doteq \begin{bmatrix}
    I \otimes \phi^T(1) \\ \vdots \\ I \otimes \phi^T(T)
    \end{bmatrix},
    B \doteq \begin{bmatrix}
    I \otimes u\gamma^T(1) \\ \vdots \\ I\otimes u\gamma^T(T)
    \end{bmatrix},
    \xi \doteq 
    \begin{bmatrix}
    y_s(1) \\ \vdots \\ y_s(T)
    \end{bmatrix}.
\end{equation}

\begin{assumption}
The consistency set $\mathcal{P}_1$ is compact. \label{assum:compact}
% ,thus enough data need to be collected until the matrix $ \begin{bmatrix} A & B \\ -A & -B \end{bmatrix}$ has full column rank. \urg{Reason?}
\end{assumption}
\begin{remark} A necessary condition for Assumption \ref{assum:compact} to hold is that $[A, B; -A, -B]$ has full column rank.
\end{remark}

\begin{remark}
The polytope $\mathcal{P}_1$ is defined by $2 nT$ linear inequality constraints. Redundant constraints may be identified and then eliminated using iterative linear programming \cite{caron1989degenerate}.
\end{remark}


\subsection{Safety Set}
The safety set $\mathcal{P}_2$, which contains all safe systems with respect to given $\mathcal{X}_0, \mathcal{X}_u$, is defined by \eqref{eq:den}. Introducing $\psi =\rho u$ to tackle the bilinearity, the safe control synthesis can be formulated as a convex optimization problem \cite{rantzer2004analysis}
\begin{subequations}\label{eq:safe_rhopsi}
\begin{align}
\nabla \cdot [\rho f + \psi g] (x)&> 0,\ \forall x\in \R^n \label{eq:safe_den} \\
|\psi(x)| &\leq c\rho(x),\ \forall x\in \R^n \label{eq:safe_u}\\
\rho (x) &> 0, \ \forall x\in \mathcal{X}_0\\
\rho (x)&\leq 0, \ \forall x\in \mathcal{X}_u,
\end{align}
\end{subequations}
where $c\geq 0$ is a given scalar.  Problem \eqref{eq:safe_rhopsi} is an infinite-dimensional \ac{LP} in the values of $(\rho, \psi)$ at each $x$, possessing both strict and non-strict inequality constraints.
\begin{remark}
Note that \eqref{eq:safe_u} is the big-M method to enforce $\psi=0$ when $\rho=0$, and it simultaneously leads to a bounded-control $|u|\leq c$ as $u=\psi/\rho$ by construction.
\end{remark}
\begin{remark}
    Constraint \eqref{eq:safe_u} may be modified to ensure that the control $u$ lies in the compact polytope $\{u \mid G u \leq h\}$ by forming the expression $G \psi \leq h (\1 \rho)$.
\end{remark}
% \begin{theorem} \label{thm:safety}
% Given an initial set $\mathcal{X}_0$ and an unsafe set $\mathcal{X}_u$, the system \eqref{eq:dynamics} is safe if there exists a scalar function $\rho(x)\in C^1$ such that
% \begin{subequations}
% \begin{align}
% \nabla \cdot [\rho (f + gu)] (x)&> 0, \ \forall x\in \R^n \label{eq:den0} \\
% \rho (x) &> 0, \ \forall x\in \mathcal{X}_0\\
% \rho (x)&\leq 0, \ \forall x\in \mathcal{X}_u.
% \end{align}
% \end{subequations}
% Further, introduce $\psi =\rho u$ to tackle the bilinearity in \eqref{eq:den0}, the safe control synthesis is formulated as a convex optimization problem
% \begin{subequations}\label{eq:safe}
% \begin{align}
% \nabla \cdot [\rho f + \psi g] (x)&> 0,\ \forall x\in \R^n \label{eq:safe_den} \\
% |\psi(x)| &\leq c\rho(x),\ \forall x\in \R^n \label{eq:safe_u}\\
% \rho (x) &> 0, \ \forall x\in \mathcal{X}_0\\
% \rho (x)&\leq 0, \ \forall x\in \mathcal{X}_u,
% \end{align}
% \end{subequations}
% \end{theorem}
% where $c$ is a scalar for the big-M relaxation to enforce $\psi=0$ if $\rho=0$. Note that \eqref{eq:safe_u} also leads to a bounded control $|u|\leq c$.
% \begin{proof}
% This follows from ... \urg{to be finished}
% \end{proof}
By the replacement $f=F\phi,g=G\gamma$ in \eqref{eq:safe_den}, the $u$-safe set $\mathcal{P}_2$ is may be described as
\begin{equation} \label{eq:p2}
    \mathcal{P}_2 \doteq \left\{\mathbf{f},\mathbf{g} \colon -
    \begin{bmatrix}
        \nabla\cdot(\rho\phi^T) & \nabla\cdot(\psi\gamma^T)
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf{f} \\ \mathbf{g}
    \end{bmatrix} < 0\right\}.
\end{equation} 

\subsection{Data-Driven Safety Control}

% Applying the Extended Farkas' Lemma to enforce $\mathcal{P}_1 \subseteq \mathcal{P}_2$ (i.e., all consistent systems are safe), leads to the main theorem of this paper.

Applying the Extended Farkas' Lemma to enforce $\mathcal{P}_1 \subseteq \mathcal{P}_2$ leads to the following lemma:
\begin{lemma}\label{lem:farkas}  
$\mathcal{P}_1 \subseteq \mathcal{P}_2$ if and only if there exists a vector function $y(x)\geq 0$ (of dimension $1\times 2nT$ where $n$ is the number of states and $T$ is the number of data) such that the following functional set of affine constraints is feasible:
\begin{equation} \label{eq:lem1}
    y(x)N = d(x) \ \text{and} \ y(x)e  \leq 0,
\end{equation} 
where for simplicity we define
\begin{equation} \begin{aligned} \label{eq:lem2}  
    & N \doteq \begin{bmatrix} A & B\\-A & -B \end{bmatrix}, \; 
    e \doteq \begin{bmatrix}\epsilon \mathbf{1} + \xi \\ \epsilon \mathbf{1} - \xi \end{bmatrix}, \\
    & d(x) \doteq - \begin{bmatrix} \nabla\cdot(\rho\phi^T) & \nabla\cdot(\psi\gamma^T) \end{bmatrix}.
\end{aligned} \end{equation}
\end{lemma}
\begin{proof}
Directly apply the Extended Farkas' Lemma.
\end{proof}

The main result of this paper is the following theorem:
\begin{theorem}\label{thm:main}
% Given noisy data of a , a sufficient condition for there to  exist 
A sufficient condition for the existence of a state-feedback control law $u(x)$ such that all $\dc$-consistent systems following system \eqref{eq:dynamics} are safe is that there exists functions $\rho \in C^1$,  $\psi\in C^0$, and a (possibly discontinuous) vector function $y(x) \geq 0$ such that
\begin{subequations}\label{eq:thm_main} 
\begin{align}
y(x)N &= d(x), \ \forall x \in \R^n\label{eq:thm_main1}\\
y(x)e  &\leq 0, \ \forall x \in \R^n\\
|\psi(x)| &\leq c\rho(x),\ \forall x\in \R^n\\
\rho(x) &> 0,\ \forall x\in\mathcal{X}_0\\ 
\rho(x) &\leq 0, \ \forall x\in\mathcal{X}_u.
\end{align}
\end{subequations}
The control law $u$ can then be extracted by the division $u(x) = \psi(x)/\rho(x)$.
% And the control law can be extracted as $u=\psi/\rho$, which is a rational polynomial function. 
\end{theorem}
\begin{proof}
Apply Lemma \ref{lem:farkas} to Problem \eqref{eq:safe_rhopsi}.
\end{proof}

\subsection{Sum-of-Squares Safety Program}
\label{sec:sos_safety}
In order to solve the infinite-dimensional Problem \eqref{eq:thm_main} in a tractable manner, we restrict the variables $\rho, \psi, y$ to be polynomials. The extracted controller $u(x) = \psi(x)/\rho(x)$ is then a rational function.
% Note that \eqref{eq:thm_main} is a feasibility polynomial problem, which can be solved using SOS program. 
Compare the coefficients $k_l, k_r$ of \eqref{eq:thm_main1} on both sides and let $\mathcal{X}_0 \doteq \{x\colon f_0(x) \geq 0\}$, $\mathcal{X}_u \doteq \{x\colon f_u(x) \geq 0\}$, a detailed algorithm is given in Alg. \ref{alg:1}.
\begin{algorithm}[h]
    \caption{Data-Driven Safe Control Design} \label{alg:1}
    \begin{algorithmic}
        \State Input: sample data $\dc$, and degrees of $f,g,\rho,\psi$.
        \State Let $d_1=\text{max}\left\{d_f+d_\rho,d_g+d_\psi \right\}, d_2 = \text{max}\left\{d_\rho,d_\psi \right\}$.
        \State Solve: the feasibility problem
        \[ \begin{array}{l}
        k_l = k_r                                 \hfill(A.1)\\
        -Ye            \; \in\Sigma_{d_1} [x]    \hfill(A.2)\\
        c\rho - \psi   \; \in \Sigma_{d_2} [x]    \hfill(A.3)\\
        c\rho + \psi   \; \in \Sigma_{d_2} [x]    \hfill(A.4)\\
        \rho - s_1f_0  \; \in \Sigma_{d_\rho} [x] \hfill(A.5)\\
        -\rho - s_2f_u \; \in \Sigma_{d_\rho} [x] \hspace{1cm}\hfill(A.6)\\
        Y_i            \; \in \Sigma_{d_1} [x]    \hfill(A.7)\\
        s_1, s_2       \; \in \Sigma_{d_2} [x]    \hfill(A.8)\\
        
        \end{array} \]
        \State Output: the safe control law $u = \psi/\rho$ or a certificate of infeasibility at the current degree 
    \end{algorithmic}
\end{algorithm}


==> sections/methods_MS.tex <==


\section{Data-Driven Safe Control} \label{sec:safe_no_w}


%%%-----------------------------
\subsection{Problem Statement}

% Consider the continuous-time control-affine system of the form
% \begin{equation} \label{eq:dynamics}
%     \dot{x} = f(x) + g(x) u
% \end{equation}
% where $x\in \R^n$ is the state, $u\in \R$ is the input, $f,g\colon \R^n \rightarrow \R^n$ are unknown polynomial functions, respectively. We assume the degrees of $f,g$ are known (or user-defined), then $f,g$ can be expressed by $f = F \phi$, $g = G \gamma$ where $F,G$ are unknown coefficient matrices and $\phi,\gamma$ are known monomial vectors in $x$, of proper dimensions. For example, for a two-state second-order polynomial system, $\phi,\gamma = [1,x_1,x_2,x_1^2,x_1x_2,x_2^2]^T$ and $F,G \in \R^{2\times 6}$.

The goal of this paper is to design a safe control law based on (noisy) experimental measurements for unknown polynomial systems where only minimal a-priori information  is available. Specifically, we consider control affine nonlinear  systems of the form
\begin{equation}\label{eq:dynamics_noise}
\dot{x}(t) = f(x) + g(x)u(t) + w(t),
\end{equation}
where the input $w$ satisfying $\forall t \geq 0 \colon w \in \mathcal{W} \subseteq \R^n$ represents an unknown random but bounded disturbance.  The only information available about the dynamics is that they can be expressed in terms of known dictionaries $\vt{\phi}({x}) \in \mathbb{R}^{s_f}, \vt{\gamma}({x}) \in \mathbb{R}^{s_g}$, that is
\beq\begin{aligned}\label{eq:pro1}
f(x) = \mt{F} \vt{\phi}({x}); \; g(x)= \mt{G} \vt{\gamma}({x}) 
\end{aligned}\eeq
for some unknown  system parameter matrices $\mt{F} \in \mathbb{R}^{n\times n_f}$ and $\mt{G} \in \mathbb{R}^{n \times n_g}$.
In this context, the problem under consideration can be formally stated as:

\begin{problem} \label{pb:1} 
% Given $T$ measurements of the triple $(\dot{x}_s, x_s, u_s)$, $s=t_1,\ldots,t_T$, 
Given  a data-collection noise bound $\epsilon>0$, a process disturbance description $w \in \mathcal{W}$ (e.g. $L_\infty$-bounded input), noisy derivative-state-input data $\dc = \{(y_s, x_s, u_s)\}_{s=t_1..t_T}$ under the relation $\norm{y_s - f(x_s) - g(x_s)u_s}_\infty \leq \epsilon$, and basic semialgebraic sets  $\mathcal{X}_0$, $\mathcal{X}_u$, find a state-feedback control law $u(x)$  that renders all closed-loop  systems consistent with the observed data and priors   robustly safe with respect to $\mathcal{X}_0$ and $\mathcal{X}_u$, for all  $w \in \mathcal{W}$.
\end{problem}

%\begin{remark}
   % The data $y_s$ is a noisy observation of the true derivative $\dot{x_s}$.
%\end{remark}

%\begin{remark}
%The solved control law $u(x)$ is not necessarily consistent with sample data $\dc$.
%\end{remark}

% In this section, we derive a data-driven algorithm to solve the problem \ref{pb:1}. 

%The data-driven Problem \ref{pb:1} will be approached by  define two polytopic sets in parameter space: one for $\dc$-consistent systems ($\mathcal{P}_1$) and one for safe systems ($\mathcal{P}_2$). Applying the Extended Farkas' Lemma to enforce set-containment leads to a polynomial feasibility problem, which can be solved with \ac{SOS} method by \ac{SDP} solvers.

\subsection{Model Based Safety} \label{sec:MBS}

In order to solve Problem \ref{pb:1}, in this section we first develop a  convex condition, less conservative than \eqref{eq:safe_rho}, that guarantees robust controlled safety of a model of the form \eqref{eq:dynamics_noise} assuming that $f(.)$ and $g(.)$ are known.

\begin{lemma}\label{lem:lemma2} Assume that the set $\mathcal{X}_u$ has a description of the form:
\[ \mathcal{X}_u \doteq \left \{x \colon h_i(x) \geq 0,\ i=1,\ldots, N_c \right \}. \]
Then, if there exist scalar functions $\rho(x), \psi(x) \in C^1$ such that: (i) $u(x) \doteq \frac{\psi(x)}{\rho(x)}$ is well defined over the safe region $\rho(x)>0$, (ii) for all $w \in \mathcal{W}$ and initial condition $x_0 \in \mathcal{X}_0$, the trajectories of \eqref{eq:dynamics_noise} are well defined, and (iii)
the following conditions hold:
\begin{subequations}\label{eq:MBS}
\begin{align}
&\nabla \cdot [\rho(x) \left(f (x) +w\right ) + \psi(x) g(x)] - \rho(x)h(x) > 0 \label{eq:MBS1} \\
& \text{$\forall x\in \R^n$ and $w \in \mathcal{W}$} \nonumber \\
&\rho (x) \geq 0, \ \forall x\in \mathcal{X}_0, \;
\rho (x)< 0, \ \forall x\in \mathcal{X}_u. 
%&u(x) \doteq \frac{\psi(x)}{\rho(x)} \; \text{bounded for all finite $x$}
\end{align}
\end{subequations}
where $h\doteq \min_i \left \{ h_i(x) \right \}$,
then the control law $u(x)$ renders the closed loop system robustly safe with respect to $\mathcal{X}_u$.
\end{lemma}
\begin{proof} Since by assumption $\rho,\psi \in C^1$ and $u$ is well defined, \eqref{eq:MBS1} is equivalent to (omit $x$):
\beq 
\frac{\partial \rho}{\partial x}(f+gu+w) + \rho \left (\nabla \cdot (f+gu) -h \right ) > 0
\eeq
where we used the fact that $\psi = \rho u$. Hence, for all $w \in \mathcal{W}$,
\[ \frac{d\rho}{dt}+ \rho\left (\nabla \cdot (f+gu) -h \right ) > 0\]
along the closed loop trajectories, which implies that $ \frac{d\rho}{dt} > 0$ when $\rho[x(t)]=0$.  Assume that there exists  a trajectory  $x(t,x_0,w)$ that starts at $x_0 \in \mathcal{X}_0$ and such that $x(T,x_0,w) \in \mathcal{X}_u$. By continuity, there exists some $0<t_1<T$ and some $dt$ such that $\rho(t_1)=0$ and $\rho(t)<0$ for all $t\in [t_1,t_1+dt]$. However, this contradicts the fact that  $\frac{d\rho}{dt} \left |_{t=t_1} > 0 \right.$.
\end{proof}
\begin{remark} Since $\min_i\left \{ h_i(x) \right \}$ has a semialgebraic representation, finding polynomial functions $\rho$ and $\psi$ reduces to 
\iac{SOS} optimization via standard 
%Putinar Positivstellensatz 
arguments.
\end{remark}
\begin{remark}  Problem \eqref{eq:MBS} is an infinite-dimensional \ac{LP} in the values of $(\rho, \psi)$ at each $x$, possessing both strict and non-strict inequality constraints. When compared against \eqref{eq:h_relaxation}, this formulation  has two advantages: (i) it avoids using an arbitrary, fixed multiplier $h(x)$, and (ii) it leads to jointly convex (in $\rho$ and $\psi$) optimization problems when searching for a control barrier and associated control action. On the other hand, \eqref{eq:MBS}, while retaining the desirable convexity properties of   \eqref{eq:safe_rho}, is less conservative: since the second term in \eqref{eq:MBS1} is nonnegative over the safe region, it does not require the first term to be positive everywhere, as is the case with  \eqref{eq:safe_rho}. Note that any feasible solution to  \eqref{eq:safe_rho} is also feasible for \eqref{eq:MBS}.
\end{remark}

\subsection{Safe Data Driven Control}\label{sec:SDDC}

This section presents the main result of the paper: a tractable, convex reformulation of Problem \ref{pb:1}.  In order to present these results, we begin by presenting  a tractable characterization of all systems that could have generated the observed data. 

Assume the sample data $\dc \doteq \left \{(y_s,x_s,u_s)\right \}$ is corrupted by a sample (offline) noise bounded by $\epsilon$. The consistency set $\mathcal{C}$, 
which contains all systems that are consistent with the data, is defined as:
\begin{equation}
    \mathcal{C} \doteq \left\{
    f,g\colon \|y_s-f(x_s)-g(x_s)u_s\|_\infty \leq \epsilon, s=t_1,\ldots,t_T \right\}.
\end{equation}
Recall that $f = \mt{F} \vt{\phi}$, $g = \mt{G} \vt{\gamma}$. Exploiting the following property of the Kronecker product \cite{petersen2008matrix} $$\text{vec}(P^TXQ^T) = (Q\otimes P^T) \text{vec}(X),$$ 
leads to the equivalent representation
\begin{equation} \label{eq:p1}
    \mathcal{C} = \left\{ 
    \vt{f},\vt{g} \colon 
    \begin{bmatrix}
        \mt{A} & \mt{B} \\ -\mt{A} & -\mt{B}
    \end{bmatrix} 
    \begin{bmatrix}
        \vt{f} \\ \vt{g}
    \end{bmatrix}
    \leq 
    \begin{bmatrix}
        \epsilon \mathbf{1} + \vt{\xi} \\ \epsilon \mathbf{1} - \vt{\xi}
    \end{bmatrix} \right\},
\end{equation}
where $\vt{f} = \text{vec} (\mt{F}^T)$, $\vt{g} = \text{vec} (\mt{G}^T)$ and
\begin{equation} \label{eq:abxi}
    \mt{A} \doteq \begin{bmatrix}
    \mt{I} \otimes \vt{\phi}^T(t_1) \\ \vdots \\ \mt{I} \otimes \vt{\phi}^T(t_T)
    \end{bmatrix},
    \mt{B} \doteq \begin{bmatrix}
    \mt{I} \otimes u\vt{\gamma}^T(t_1) \\ \vdots \\ \mt{I} \otimes u\vt{\gamma}^T(t_T)
    \end{bmatrix},
    \vt{\xi} \doteq 
    \begin{bmatrix}
    y(t_1) \\ \vdots \\ y(t_T)
    \end{bmatrix}.
\end{equation}

%\begin{assumption}
%The consistency set $\mathcal{C}$ is compact. %\label{assum:compact}
% ,thus enough data need to be collected until the matrix $ \begin{bmatrix} A & B \\ -A & -B \end{bmatrix}$ has full column rank. \urg{Reason?}
%\end{assumption}
%\begin{remark} A necessary condition for Assumption \ref{assum:compact} to hold is that $[A, B; -A, -B]$ has full column rank.
%\end{remark}
In order to establish robust safety, we need to add to this representation a description of all admissible disturbances. In the sequel, we will assume that this set  has a polytopic description of the form $\mathcal{W} \doteq \left \{ \vt{w} \colon \mt{W} \vt{w} \leq \vt{d}_w \right \}$. Combining this description with the description of $\mathcal{C}$ leads to an augmented consistency set describing the set of all possible plants and disturbances:
\begin{equation}\label{eq:P1}
    \mathcal{P}_1 \doteq \left\{ \vt{f,g,w} \colon
    \begin{bmatrix}
        \mt{A} & \mt{B} & 0\\
        -\mt{A} & -\mt{B} & 0\\
        0 & 0 & \mt{W}
    \end{bmatrix}
    \begin{bmatrix}
        \vt{f}\\ \vt{g} \\ \vt{w}
    \end{bmatrix}
    \leq 
    \begin{bmatrix}
        \epsilon \mathbf{1} + \xi\\
        \epsilon \mathbf{1} - \xi\\
        \vt{d}_w\\
        \end{bmatrix} \right\}.
\end{equation}


%\begin{remark}
%The polytope $\mathcal{P}_1$ is defined by $2 nT + n_w$ linear %inequality constraints. Redundant constraints may be eliminated %using iterative linear programming \cite{caron1989degenerate}.
%\end{remark}

It follows that a pair $(\rho,\psi)$ solves Problem \ref{pb:1} if 
\beq \label{eq:allfgw}
\nabla \cdot [\rho f (x) + \psi g(x) + \rho w] - \rho(x)h(x)> 0 \eeq
holds for all $x$ and all $(\vt{f},\vt{g},\vt{w}) \in \mathcal{P}_1$. In principle, this condition can be reduced to an \ac{SOS} optimization over the coefficients of $\rho,\psi$ by a straight application of Putinar's Positivstellensatz. However, this approach quickly becomes intractable, since it requires considering polynomials in the indeterminates $(\vt{x},\vt{f},\vt{g},\vt{w})$ with a total dimension $n_p=n_f+n_g+2n$. Thus, for a relaxation of order $n_r$ the total number of variables in the optimization is
$\binom{n_r+n_p}{n_p}$. As an example,  for a second order system with polynomial dynamics of degree 2, we have $n_f =n_g=6$. If $\rho$ and $\psi$ are also limited to degree 2 polynomials, a relaxation of order $n_r=3$ involves 969 variables.  As we show next, computational complexity can be substantially reduced by exploiting duality. 

For a given pair $(\rho,\psi)$, consider the set of all systems of the form \eqref{eq:dynamics_noise} that are rendered safe by the control action $u=\frac{\psi}{\rho}$, along with the corresponding admissible perturbations, that is, the set of all
$(\vt{f},\vt{g},\vt{w})$ such that \eqref{eq:allfgw} holds for all $x \in \R^n$. For each $x$, this set is a polytope of the form:
\begin{equation}
    \mathcal{P}_2 \doteq \left\{\vt{f},\vt{g},\vt{w}\colon -
    \begin{bmatrix}
        (\nabla\cdot(\rho\phi^T))^T \\  
        (\nabla\cdot(\psi\gamma^T))^T\\
        (\nabla\rho)^T
    \end{bmatrix}^T
    \begin{bmatrix}
        \vt{f} \\ \vt{g} \\ \vt{w}
    \end{bmatrix} < -\rho h\right\}.
\end{equation}

It follows that \eqref{eq:allfgw} holds for all admissible disturbances $\vt{w} \in \mathcal{W}$ and all plants in the consistency $\mathcal{C}$ set if and only if $\mathcal{P}_1 \subseteq \mathcal{P}_2$.  This inclusion can be enforced through duality as follows:
%the extended Farkas' Lemma as follows:

\begin{lemma}\label{lem:farkas}   Assume that the data and priors are consistent (e.g. $\mathcal{C} \not = \emptyset$) and that  enough data has been collected so that $\mathcal{C}$ is compact. Then 
$\mathcal{P}_1 \subseteq \mathcal{P}_2$ if and only if there exists a vector function $\vt{y}(x)\geq 0, \vt{y}(x) \in \R^{2nT+2n}$ such that the following functional set of affine constraints is feasible:
\begin{equation}\label{eq:EFL}
    \vt{y}^T(x) \mt{N} = \vt{r}(x) \; \text{and} \;
    \vt{y}^T(x) \vt{e}  < -\rho(x)h(x)
\end{equation}
where
\begin{equation}
    \begin{aligned} \label{eq:Ndef}  & \mt{N} \doteq 
    \begin{bmatrix}
    \mt{A} & \mt{B} & 0\\
    -\mt{A} & -\mt{B} & 0 \\
    0 & 0 & \mt{W}\\
    \end{bmatrix}, 
    \; \vt{e} \doteq 
    \begin{bmatrix}
        \epsilon \mathbf{1} + \vt{\xi}\\
        \epsilon \mathbf{1} - \vt{\xi}\\
      \vt{d}_w
    \end{bmatrix}, \\
    & \vt{r}(x)\doteq -
    \begin{bmatrix}
        \nabla\cdot(\rho\vt{\phi}^T) & \nabla\cdot(\psi\vt{\gamma}^T) & \nabla\rho
    \end{bmatrix}.
    \end{aligned}
\end{equation}
\end{lemma}
\begin{proof} Since $\mathcal{C}$ is compact, from section 5.8.3 in \cite{boyd2004convex} it follows that the systems of inequalities
\beq \label{eq:alternatives}
  %  \begin{aligned}
       \begin{bmatrix} \mt{N} \\ -\vt{r} \end{bmatrix}  \begin{bmatrix}
        \vt{f} \\ \vt{g} \\ \vt{w}
    \end{bmatrix} \leq \begin{bmatrix} \vt{e} \\ \rho(x)h(x) \end{bmatrix} \; \textrm{and} \;\begin{array}{r}
    \vt{y}^T\mt{N}-\mu \vt{r} = 0 \\
     \vt{y}^T\vt{e} + \mu \rho(x)h(x) < 0 \\
    \vt{y} \geq 0, \; \mu \geq 0
    \end{array}
   % \end{aligned}
\eeq
are strong alternatives. Further, since $\mathcal{C} \not = \emptyset$ and $\mu >0$, we can take $\mu=1$ without loss of generality. Thus \eqref{eq:EFL} holds if and only if the left set of inequalities in \eqref{eq:alternatives} is infeasible. This implies that if \eqref{eq:EFL} holds,  a triple $(\vt{f,g,w}) \in \mathcal{P}_1$ if and only if 
$\begin{bmatrix}\vt{f}^T\; \vt{g}^T\;\vt{w}^T \end{bmatrix} \vt{r}^T < -\rho(x)h(x) $, that is  $(\vt{f,g,w}) \in \mathcal{P}_2$.
%Follows from direct application of the Extended Farkas' Lemma.
\end{proof}
\begin{remark} Proceeding as in Theorem 2 in \cite{dai2020semi}, it can be shown that  if $\vt{\phi}(\mat{x}), \vt{\gamma}(\mat{x})$ are continuous functions, then $\vt{y}({x})$ can be chosen to be continuous.
%\textcolor{red}{Further, if  $\vt{\phi},\vt{\gamma},\rho,\psi$ are polynomial and the trajectories of the closed-loop system stay in a compact region, then, without loss of generality $\vt{y}({x})$  can be taken to be polynomial. 
\end{remark}

Combining the observations above leads to
the main result of this paper:
\begin{theorem}\label{thm:main}
% Given noisy data of a , a sufficient condition for there to  exist 
A sufficient condition for the existence of a state-feedback control law $u(x)$ such that all systems in the consistency set $\mathcal{C}$ are rendered robustly safe, is that there exists a continuous vector function $\vt{y}(x) \geq 0$ and functions $\rho \in C^1$, $\psi\in C^1$ 
%with $\frac{\psi(x)}{\rho(x)} \in C^0$
such that
\begin{subequations}\label{eq:thm_main} 
\begin{align}
\vt{y}^T(x)\mt{N} &= \vt{r}(x), \ \forall x \in \R^n\label{eq:thm_main1}\\
\vt{y}^T(x)\vt{e}  & < -\rho(x)h(x), \ \forall x \in \R^n \label{eq:thm_main2}\\
|\psi(x)| &\leq -\rho(x)h(x),\ \forall x\in \R^n \label{eq:thm_main3}\\
\rho(x) & \geq 0,\ \forall x\in\mathcal{X}_0\\ 
\rho(x) & < 0, \ \forall x\in\mathcal{X}_u.
\end{align}
\end{subequations}
The control law $u$ can then be extracted by the division $u(x) = \psi(x)/\rho(x)$.
% And the control law can be extracted as $u=\psi/\rho$, which is a rational polynomial function. 
\end{theorem}
\begin{proof} The proof follows from the fact that from Lemma \ref{lem:farkas}, \eqref{eq:thm_main1} and \eqref{eq:thm_main2} guarantee that \eqref{eq:allfgw} holds for all plants in $\mathcal{C}$ and all admissible disturbances $\vt{w} \in \mathcal{W}$. Hence the conditions in Lemma \ref{lem:lemma2} hold for all plants that could have generated the observed data.
\end{proof}
    
\begin{remark}
Note that \eqref{eq:thm_main3} is a convex tightening of the condition that $\psi=0$ when $\rho=0$, %Simultaneously, it  leads to a bounded-control $|u|\leq c$ as $u=\psi/\rho$ by construction.
and for the safety concern, we focus on the region where it is safe.
\end{remark}

\subsection{Sum-of-Squares Safety Program}
\label{sec:sos_safety}
In order to solve the infinite-dimensional Problem \eqref{eq:thm_main} in a tractable manner, we restrict the variables $\rho, \psi, \vt{y}$ to be polynomials. Under this polynomial restriction, the extracted controller $u(x) = \psi(x)/\rho(x)$ is then a rational function.
% Note that \eqref{eq:thm_main} is a feasibility polynomial problem, which can be solved using SOS program. 



% . The set of \ac{SOS} polynomials is a strict subset of all nonnegative polynomials, but 

% \subsection{SOS Polynomials}
% This paper shows that the data-driven safe control synthesis can be formulated as a polynomial nonnegativity  problem, which is generally NP-hard (for polynomials of even degree $d\geq 4$). This difficulty can be handled by relaxing the problem to establishing that a given polynomial is a Sum of Squares. Consider a polynomial $f$ of degree $2m$. A sufficient condition to $\forall x \in \R^n: f(x)\geq 0$ is that $f$ can be written as a \ac{SOS} 
% $f = \textstyle \sum_i g_i^2.$
% Let $v$ be a vector with all monomials of degree less than or equal to $m$. Then $f$ is \ac{SOS} if and only if there exists a positive semidefinite matrix $Q$ such that
% $f = v^T Qv$ \cite{parrilo2000structured}.
% Comparing term on the both sides leads to an \ac{SDP} program, which can be solved by off-the-shelf solvers. \textcolor{red}{do we need to mention the Psatz?}


Let $\mathcal{X}_0 \doteq \{x\colon k(x) \geq 0\}$ and $\mathcal{X}_u \doteq \{x\colon h(x) \geq 0\}$ denote the initial condition and unsafe sets, respectively. Algorithm 1 is \iac{SOS}-based finite-degree tightening of \eqref{eq:thm_main} for robustly safe control. Successful execution of algorithm \ref{alg:1} is sufficient for finding a robustly safe control law. 
%\urg{note that (A.2) imposes non-negativity instead of positivity}
% a detailed algorithm for data-driven robustly safe control is given in Alg. \ref{alg:1}.
\begin{algorithm}[h]
    \caption{Data-Driven Safe Control Design} \label{alg:1}
    \begin{algorithmic}
        \State Input: sample data $\dc$, and degrees of $f,g,\rho,\psi$
        \State Let 2$d_1\geq\text{max}\left\{d_f+d_\rho,d_g+d_\psi \right\}, 2d_2 \geq \text{max}\left\{d_\rho,d_\psi \right\}$
        \State Solve: the feasibility problem
        \[ \begin{array}{rcl}
        \textrm{coeff}_x(\vt{y}^T(x) \mt{N} - \vt{r}(x))&=0                              \hfill(A.1) \\
        -\rho(x)h(x) - \vt{y}^T(x) \vt{e} - c_1\; &\in \Sigma_{d_1}[x] \hspace{1cm}   \hfill(A.2)\\
        -h\rho - \psi   \; &\in \Sigma_{d_2}[x]   \hfill(A.3)\\
        -h\rho + \psi   \; &\in \Sigma_{d_2}[x]   \hfill(A.4)\\
        \rho - s_1k  \; &\in \Sigma_{d_2} [x]  \hfill(A.5)\\
        -\rho - s_2h - c_2\; &\in \Sigma_{d_2} [x]  \hfill(A.6)\\
        \vt{y}_i            \; &\in \Sigma_{d_1}[x]    \hfill(A.7) \\
        c_1, c_2       \; &> 0    \hfill(A.8) \\
        s_1, s_2       \; &\in \Sigma_{d_2}[x]    \hfill(A.9)\\
        \end{array} \]
        \State Output: the safe control law $u = \psi/\rho$ or a certificate of infeasibility at degree $(d_1, d_2)$ 
    \end{algorithmic}
\end{algorithm}

% \urg{note about lack of convergence guarantee?}

==> sections/preliminaries.tex <==
\section{Preliminaries} \label{sec:preliminaries}

% \subsection{Acronyms/Initialisms}
\input{sections/acronym}

\subsection{Notation} \label{subsec:notation}

\begin{tabular}{p{0.13\columnwidth}p{0.75 \columnwidth}}
$\R^n$ & Set of $n$-tuples of real numbers\\
$x,X,I$ & Vector, matrix, identity matrix\\
$\mathbf{1,0}$ & Vector/matrix of all 1s, 0s\\
$\left\|x \right\|_p$ & $\ell_p$-norm of vector $x$\\
$\left\|X \right\|_p$ & Induced $\ell_p$-norm of matrix $X$\\
$X\succeq 0$ & $X$ is positive semi-definite \\
$\otimes$ & Kronecker product\\
\text{vec}$(X)$ & Vectorized matrix along columns: \\ & $\text{vec}(X)= \left[ X(\colon,1)^T,\cdots,X(\colon,n)^T\right]^T$ \\
$\rho \in C^d$ & $\rho$ has a continuous $d^{th}$ derivative\\
$\nabla \rho$ & Gradient of scalar function $\rho$ \\
$\nabla \cdot f$ & Divergence of vector function $f$\\
$\Sigma[x]$ & Cone of \ac{SOS} polynomials in $x \in \R^n$
\end{tabular}

% \begin{itemize}
%     \item[A1] Assumption 1
%     \item[A2]  Assumption 2
% \end{itemize}

\subsection{Safe Systems}
Consider the continuous-time control-affine system of the form\footnote{For notational simplicity, single-input systems are considered, but the result can be extended to multi-input systems trivially.}
\begin{equation} \label{eq:dynamics}
    \dot{x} = f(x) + g(x) u,
\end{equation}
where $x\in \R^n$ is the state, $u\in \R$ is the control input, and $f,g$ are unknown vector-valued polynomial functions of dimension $n\times 1$. Let $f = F \phi$, $g = G \gamma$ (with $x$ omitted), where $F,G$ are unknown coefficient matrices and $\phi,\gamma$ are known monomial vectors. For example, a two-state second-order polynomial system could have $\phi,\gamma = [1,x_1,x_2,x_1^2,x_1x_2,x_2^2]^T$ and $F,G \in \R^{2\times 6}$ in the standard monomial basis.
\begin{definition}
Given an initial set $\mathcal{X}_0$ and an unsafe set $\mathcal{X}_u$, a system is safe under the control law $u$ if there exists no trajectory starting within $\mathcal{X}_0$ will enter $\mathcal{X}_u$ as $t\geq 0$.
\end{definition}
\begin{theorem}[\cite{rantzer2004analysis}] \label{thm:safety}
Given $\mathcal{X}_0$ and $\mathcal{X}_u$, system \eqref{eq:dynamics} is safe if there exists a scalar function $\rho(x)\in C^1$ such that
\begin{subequations} \label{eq:safe_rhou}
\begin{align}
\nabla \cdot [\rho (f + gu)] (x)&> 0, \ \forall x\in \R^n \label{eq:den} \\
\rho (x) &> 0, \ \forall x\in \mathcal{X}_0\\
\rho (x)&\leq 0, \ \forall x\in \mathcal{X}_u.
\end{align}
\end{subequations}
\end{theorem}
% \begin{theorem}
%     If the integrability condition $\int_{\R^n} \rho(x) dx < \infty$ holds in addition to \eqref{eq:safe_rhou}, then $x=0$ is asymptotically stable for all $x$ originating in $\mathcal{X}_0$ \urg{get the right source and denominator for this, if we use rational polynomials}
% \end{theorem}

% \begin{proof}
% This follows from ... \urg{to be finished}
% \end{proof}




%%%-------------------------------------------------
% \subsection{Farkas' Lemma (variant)}

% \begin{lemma}
% Let $A\in \R^{m\times n}$ and $b\in \R^n$. Then the following statements are strongly alternative, i.e., exactly one of them is true:
% \begin{enumerate}
%     \item There exists an $x\in \R^n$ such that $Ax \leq b$.
%     \item There exists a $y\geq 0, y\in\R^m$ such that $A^T y = 0$ and $b^T y <0$.
% \end{enumerate}
% \end{lemma}
%%%-------------------------------------------------

\subsection{Extended Farkas' Lemma}
This work attempts to find a state-feedback control law such that the set of all consistent systems is contained in the set of all safe systems. Such set-containment is enforced by using the Extended Farkas' Lemma:
\begin{lemma}[\cite{hennet1989farkas, henrion1999control}]
Consider polytopes $\mathcal{P}_1 =\left\{ x| A_1 x \leq b_1 \right\}$ and $\mathcal{P}_2 =\left\{ x| A_2 x \leq b_2 \right\}$. Then $\mathcal{P}_1 \subseteq \mathcal{P}_2$ if and only if there exists a nonnegative matrix $Y$ of appropriate dimensions such that
$$Y A_1= A_2\ \text{and} \ Y b_1 \leq b_2.$$
\end{lemma}


% \subsection{Kronecker Product}
% Let $A\in \R^{m\times n}$ and $B\in \R^{p\times q}$, the Kronecker product $A\otimes B$ is the $\R^{mp\times nq}$ matrix:\\
% $$A\otimes B = \begin{bmatrix} 
% a_{11} B & \cdots & a_{1n} B \\
% \vdots & \ddots & \vdots \\
% a_{m1} B & \cdots & a_{mn} B 
% \end{bmatrix}, $$
% and the following property will be used in this paper
% \begin{equation} \label{eq:kron}
%     \text{vec}(B^TX^TA^T) = (A\otimes B^T) \text{vec}(X^T).
% \end{equation}

\subsection{SOS Polynomials}
This paper shows that the data-driven safe control synthesis can be formulated as a polynomial feasibility problem, which is generally NP-hard (for polynomials of even degree $d\geq 4$). To tackle this, \ac{SOS} polynomials are used as a convex relaxation for nonnegative polynomials. Consider a polynomial $f$ of degree $2m$. A sufficient condition to $\forall x \in \R^n: f(x)\geq 0$ is that $f$ can be written as a sum of squares of polynomials $g_i$ of degree $m$:
$f = \textstyle \sum_i g_i^2.$
Let $v$ be a vector with all monomials of degree less than or equal to $m$. Then $f$ is \ac{SOS} if and only if there exists a positive semidefinite matrix $Q$ such that
$f = v^T Qv.$
Comparing term on the both sides leads to an \ac{SDP} program, which can be solved by off-the-shelf solvers.

